Modeling the Galaxy Distribution in Clusters using Halo Cores

The galaxy distribution in dark matter-dominated halos is expected to approximately trace the details of the underlying dark matter substructure. In this paper we introduce halo `core-tracking' as a way to efficiently follow the small-scale substructure in cosmological simulations and apply the technique to model the galaxy distribution in observed clusters. The method relies on explicitly tracking the set of particles identified as belonging to a halo's central density core, once a halo has attained a certain threshold mass. The halo cores are then followed throughout the entire evolution of the simulation. The aim of core-tracking is to simplify substructure analysis tasks by avoiding the use of subhalos and, at the same time, to more easily account for the so-called ``orphan'' galaxies, which have lost substantial dark mass due to tidal stripping. We show that simple models based on halo cores can reproduce the number and spatial distribution of galaxies found in optically-selected clusters in the Sloan Digital Sky Survey. We also discuss future applications of the core-tracking methodology in studying the galaxy-halo connection.

==> hyperlink-year-only-natbib-patch.tex <==
% found on https://tex.stackexchange.com/questions/23227/how-to-hyperlink-only-the-year-part-when-using-natbib-and-hyperref

\RequirePackage{hyperref}
\RequirePackage{natbib}
\RequirePackage{etoolbox}

\makeatletter

% Patch case where name and year are separated by aysep
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@aysep\NAT@spacechar}{\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@aysep\NAT@spacechar\NAT@hyper@{\NAT@date}}{}{}

% Patch case where name and year are separated by opening bracket
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi}%
       {\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi\NAT@hyper@{\NAT@date}}
  {}{}

\makeatother

